Congestion Mitigation Path Planning for Large-Scale Multi-Agent Navigation in Dense Environments

In high-density environments where numerous autonomous agents move simultaneously in a distributed manner, streamlining global flows to mitigate local congestion is crucial to maintain overall navigation efficiency. This paper introduces a novel path-planning problem, congestion mitigation path planning (CMPP), which embeds congestion directly into the cost function, defined by the usage of incoming edges along agents' paths. CMPP assigns a flow-based multiplicative penalty to each vertex of a sparse graph, which grows steeply where frequently-traversed paths intersect, capturing the intuition that congestion intensifies where many agents enter the same area from different directions. Minimizing the total cost yields a set of coarse-level, time-independent routes that autonomous agents can follow while applying their own local collision avoidance. We formulate the problem and develop two solvers: (i) an exact mixed-integer nonlinear programming solver for small instances, and (ii) a scalable two-layer search algorithm, A-CMTS, which quickly finds suboptimal solutions for large-scale instances and iteratively refines them toward the optimum. Empirical studies show that augmenting state-of-the-art collision-avoidance planners with CMPP significantly reduces local congestion and enhances system throughput in both discrete- and continuous-space scenarios. These results indicate that CMPP improves the performance of multi-agent systems in real-world applications such as logistics and autonomous-vehicle operations.

==> table-lifelong-mapf_runtime_limit.tex <==
{
\renewcommand{\arraystretch}{0.9}
\begin{table}[t]
\centering
\caption{Throughput improvements (\%) relative to baseline (without CMPP) when varying A-CMTS runtime limit $t_L$ (\si{\second}). The raw throughput values are shown in parentheses.}
\label{table:A_CMTS-runtime}
\begin{tabular}{@{}crrr@{}}
\toprule
Map & \multicolumn{1}{c}{$|A|$} & \multicolumn{1}{c}{$t_L = 0.1$} & \multicolumn{1}{c}{$t_L = 1.0$} \\ \midrule
\multirow{3}{*}{\textit{small warehouse}} & 100 & 22.9 (4.28) & \textbf{23.6 (4.31)} \\
 & 200 & 40.7 (5.50) & \textbf{41.8 (5.55)} \\
 & 300 & 15.9 (5.05) & \textbf{17.1 (5.10)} \\ \midrule
\multirow{3}{*}{\textit{medium warehouse}} & 400 & 42.3 (7.13) & \textbf{43.9 (7.21)} \\
 & 600 & 41.6 (7.70) & \textbf{42.8 (7.76)} \\
 & 800 & \textbf{24.9 (7.43)} & \textbf{24.9 (7.43)} \\ \bottomrule
\end{tabular}
\end{table}
}
